Beyond Plain Toxic: Detection of Inappropriate Statements on Flammable Topics for the Russian Language

Toxicity on the Internet, such as hate speech, offenses towards particular users or groups of people, or the use of obscene words, is an acknowledged problem. However, there also exist other types of inappropriate messages which are usually not viewed as toxic, e.g. as they do not contain explicit offences. Such messages can contain covered toxicity or generalizations, incite harmful actions (crime, suicide, drug use), provoke "heated" discussions. Such messages are often related to particular sensitive topics, e.g. on politics, sexual minorities, social injustice which more often than other topics, e.g. cars or computing, yield toxic emotional reactions. At the same time, clearly not all messages within such flammable topics are inappropriate. Towards this end, in this work, we present two text collections labelled according to binary notion of inapropriateness and a multinomial notion of sensitive topic. Assuming that the notion of inappropriateness is common among people of the same culture, we base our approach on human intuitive understanding of what is not acceptable and harmful. To objectivise the notion of inappropriateness, we define it in a data-driven way though crowdsourcing. Namely we run a large-scale annotation study asking workers if a given chatbot textual statement could harm reputation of a company created it. Acceptably high values of inter-annotator agreement suggest that the notion of inappropriateness exists and can be uniformly understood by different people. To define the notion of sensitive topics in an objective way we use on guidelines suggested commonly by specialists of legal and PR department of a large public company as potentially harmful.

==> comparison-of-binary-and-pairwise.tex <==
\subsection{Comparison of Annotation Schemes: Binary vs Pairwise}


The most straightforward way to get the binary annotation is to ask an annotator whether a given sample is appropriate or not as it is shown in Figure~\ref{fig:binary_interface}. Alternatively, we can ask which of the two samples is less appropriate (see Figure~\ref{fig:pairwise_interface}) and then aggregate the comparisons into a ranking. This way is useful in cases when it is difficult to make a binary decision, which can happen in our task where many examples belong to the ``gray area'' between the definitely appropriate and absolutely inappropriate.

\subsubsection{Experimental Setup}

The aim of comparison of binary annotation and pairwise comparison approaches is to determine which of them is (i)~easier for workers, (ii)~more accurate, (iii)~better scalable for larger amount of data, and (iv)~cheaper.
Thus, we pick 1,000 samples from the multilabel dataset, keeping the balance of the sensitive topics. We label it twice: via binary and pairwise annotation.
We then evaluate the two approaches by comparing their performance on a test set. We randomly select 200 sentences from the 1,000 examples and label them manually. The quality of a crowdsourced annotation approach is defined as its accuracy with respect to this manual expert annotation.


We perform the \textit{binary annotation} with the average overlap of 4. The overlap for an individual example is defined dynamically as described in Section \ref{sec:crowdsourcing}. The average performance of workers on the training and control tasks is 80\%. In terms of this experiment this fact is enough to roughly assume that the notion of inappropriateness could be understood by the workers in a uniform way. %However, on this stage it is not a mathematically proven fact, but it is enough for revealing the strong side of the binary annotation setup in terms of its comparison with pairwise setup. %This fact indicates that the notion of inappropriateness is understood by the workers in a uniform way, although it was not defined explicitly.


For \textit{pairwise annotation} we first manually label samples as appropriate / undefined / inappropriate to create the initial ranking. We then apply LUCBRank algorithm~\cite{pmlr-v84-katariya18a}. This algorithm serves for coarse ranking, i.e. distributing objects into several clusters with respect to some characteristic (in our case, the level of inappropriateness). It creates the ranking based on the similarity of objects and their level of uncertainty. Then, the ranking is refined by getting ground-truth comparisons of pairs of objects with the higher uncertainty which are likely to be misclassified. We use LUCBRank for selecting the most informative pairs for further annotation.

We label the pairs in Yandex.Toloka using the same setup as before. After annotation we aggregate the comparisons into ranking. We test three aggregation approaches: Bradley-Terry~\cite{BradleyTerry} (iterative algorithm which assigns a number from 0 to 1 to each sample based on its comparisons with other samples), I-LSR~\cite{Maystre2015} (the variation of Bradley-Terry model computed via maximum-likelihood inference), and LUCBRank~\cite{pmlr-v84-katariya18a} (there, the ranking is estimated after each comparison, so there is no dedicated aggregation stage). Following Bugakova et al.~\cite{Bugakova2019}, we evaluate the performance of aggregation models with the number of comparisons which are correctly reflected in the rankings by different methods (i.e. comparisons where the better item has a higher rank). The I-LSR algorithm shows the best result. Finally, we convert the ranking into binary scores using the formula $1 - \frac{r}{N}$, where $N$ is the overall number of samples and $r$ is the sample's rank.

\subsubsection{Results and Discussions}

We compute the accuracies of binary and pairwise annotations with respect to the manual annotation of 200 test samples. The accuracies are 0.84 for binary annotation and 0.83 for pairwise annotation, which suggests that they are equal in terms of annotation quality. Therefore, in order to define the preferred annotation type we analyse other parameters.

\begin{table}[ht!]
\centering
\begin{tabular}{l|l|l}
\toprule
                          & \textbf{Binary annotation}                                                                                                               & \textbf{Pairwise annotation}                                                                                             \\ \toprule
Task difficulty & \cellcolor{red!25}Decision is not evident                                                                                       & \cellcolor{green!25}Evident in most of the cases                                                                         \\ \midrule
User bias                 & \cellcolor{red!25}Present                                                                                                              & \cellcolor{green!25}Almost eliminated                                                                                    \\ \midrule
Topic bias & \cellcolor{green!25}Can be controlled  & \cellcolor{red!25} Present \\ \midrule
%annotation cost per HIT     & \cellcolor{green!25}\$0.002                                                                                                                  &     \$0.002 \cellcolor{green!25}                                                                                                \\ \midrule
\begin{tabular}[c]{@{}l@{}}Annotation cost \\ per sample\end{tabular}  & \cellcolor{green!25}Constant                                                                                                             &  \cellcolor{red!25} Goes up as the dataset grows                                                                                                   \\ \midrule
Pre-processing            & \cellcolor{green!25}Trivial                                                                                                              & \cellcolor{red!25}Pre-ranking, selection of pairs                                                                      \\ \midrule
Post-processing           &\cellcolor{green!25} \begin{tabular}[c]{@{}l@{}}Aggregation of multiple \\ answers per sample \\(implemented in \\Yandex.Toloka)\end{tabular} &\cellcolor{red!25} \begin{tabular}[c]{@{}l@{}}Aggregation of comparisons \\ into ranking \\ (not implemented in any known \\to us crowdsourcing paltform)\end{tabular} \\ \midrule
Accuracy                  & \cellcolor{green!25}0.84                                                                                                                 & \cellcolor{green!25}0.83                                                                                                 \\ \bottomrule
Final decision            &  \cellcolor{green!25}~~\ding{52}                                                                                                                   & \cellcolor{red!25}~~\ding{56}     \\                                             \bottomrule                                                  
\end{tabular}
\caption{Comparison of properties of binary and pairwise annotation setups. Better values are highlighted with green, worse values are shown in red.}
\label{table:pairwise_binary}
\end{table}

The manual analysis of pairwise annotation reveals the \textbf{topic bias}: samples on topics with higher probability to yield a toxic conversation (e.g. murder, terrorism) are ranked higher than topics where the probability of getting a severely toxic message is lower (e.g. downloading content from torrent, alcohol). 
It also occasionally emerges in binary annotation setup when samples on from both of the aforementioned groups are mixed at the same task page.
However, this topic bias is not inherent to binary annotation setup. It can be controlled by careful selection of topics in an annotation pool.
 
Another weak point of pairwise annotation is \textbf{greater cost} which is \textbf{more difficult to predict}, because in pairwise annotation the number of required comparisons per sample grows as we add more samples. This makes the \textbf{extension of dataset difficult}, because it becomes more expensive for larger datasets. 
In addition to that, to ensure the high quality of pairwise annotation, we need to perform \textbf{laborious preprocessing}, i.e. categorize all samples into inappropriate/undefined/appropriate.

Table~\ref{table:pairwise_binary} summarizes the comparison of binary and pairwise annotation setups. It shows the discussed properties of the two approaches and highlights the more favourable value with green and the less favourable one with red. The cost of pairwise annotation (both actual cost and the cost of potential dataset extension) is higher. Besides that, pairwise annotation is more difficult to set up and requires more pre- and post-processing. Since this is not compensated with higher quality (the quality of the approaches is the same), we decide to perform the rest of annotation using binary setup.

